Cohomology fractals

We introduce cohomology fractals; these are certain images associated to a cohomology class on a hyperbolic three-manifold. They include images made entirely from circles, and also images with no geometrically simple features. They are closely related to limit sets of kleinian groups, but have some key differences. As a consequence, we can zoom in almost any direction to arbitrary depth in real time. We present an implementation in the setting of ideal triangulations using ray-casting.

==> header_article.tex <==
%%% Environments %%%

% Numbering
% see http://tex.stackexchange.com/questions/41299/how-to-identify-the-counter-of-equation-theorem-and-section

\makeatletter
\let\c@equation\c@subsection
\makeatother
\numberwithin{equation}{section} 

\makeatletter
\let\c@figure\c@equation
\makeatother
\numberwithin{figure}{section} 

% Formatting 
% see amsthdoc.pdf for general discussion. 

% \swapnumbers 

% It is Bourbaki style to put labels (numbering) before the <type>.
% This is used in various places - eg Dunfield recently, Bridson and
% Haefliger.  Suggested, but not used, by Bernstein
% (http://cr.yp.to/writing.html).  If you fix the non-bold/bold/italic
% problem (three typefaces in three words arrgh!) then it looks
% better.  But it doesn't match usage in the text, and I think that
% controls...  Perhaps if the numbers could be placed in the margin in
% a nice way?  But then there wuld be a ragged left.

\theoremstyle{plain}
\newtheorem{theorem}[equation]{Theorem}
\newtheorem{corollary}[equation]{Corollary}
\newtheorem{lemma}[equation]{Lemma}
\newtheorem{conjecture}[equation]{Conjecture}
\newtheorem{proposition}[equation]{Proposition}
\newtheorem{principle}[equation]{Principle}
\newtheorem{axiom}[equation]{Axiom}
\newtheorem{ourrule}[equation]{Rule}

\theoremstyle{definition}
\newtheorem{definition}[equation]{Definition}
\newtheorem{problem}[equation]{Problem}
\newtheorem{solution}[equation]{Solution}
\newtheorem{exercise}[equation]{Exercise}
\newtheorem{example}[equation]{Example}
\newtheorem{fact}[equation]{Fact}
\newtheorem{question}[equation]{Question}
\newtheorem*{question*}{Question}
\newtheorem*{answer*}{Answer}
\newtheorem*{application*}{Application}
\newtheorem{algorithm}[equation]{Algorithm}
\newtheorem{objective}{Objective}[section]

\theoremstyle{remark}
\newtheorem{remark}[equation]{Remark}
\newtheorem*{remark*}{Remark}
\newtheorem{remarks}[equation]{Remarks}
\newtheorem{case}{Case}
\newtheorem*{case*}{Case}
\renewcommand{\thecase}{\Roman{case}}
\newtheorem{claim}[equation]{Claim}
\newtheorem*{claim*}{Claim}
\newtheorem*{proofclaim}{Claim}
\newtheorem*{proofsubclaim}{Subclaim}

%%% Refs
\newcommand{\refsec}[1]{Section~\ref{Sec:#1}}
\newcommand{\refapp}[1]{Appendix~\ref{App:#1}}
\newcommand{\refthm}[1]{Theorem~\ref{Thm:#1}}
\newcommand{\refcor}[1]{Corollary~\ref{Cor:#1}}
\newcommand{\reflem}[1]{Lemma~\ref{Lem:#1}}
\newcommand{\refprop}[1]{Proposition~\ref{Prop:#1}}
\newcommand{\refclm}[1]{Claim~\ref{Clm:#1}}
\newcommand{\refrem}[1]{Remark~\ref{Rem:#1}}
\newcommand{\refexa}[1]{Example~\ref{Exa:#1}}
\newcommand{\reffac}[1]{Fact~\ref{Fac:#1}}
\newcommand{\refexe}[1]{Exercise~\ref{Exe:#1}}
\newcommand{\reffig}[1]{Figure~\ref{Fig:#1}}
\newcommand{\reftab}[1]{Table~\ref{Tab:#1}}
\newcommand{\refdef}[1]{Definition~\ref{Def:#1}}
\newcommand{\refprob}[1]{Problem~\ref{Prob:#1}}
\newcommand{\refalg}[1]{Algorithm~\ref{Alg:#1}}
\newcommand{\refax}[1]{Axiom~\ref{Ax:#1}}
\newcommand{\refrul}[1]{Rule~\ref{Rul:#1}}
\newcommand{\refeqn}[1]{Equation~\ref{Eqn:#1}}
\newcommand{\refconj}[1]{Conjecture~\ref{Conj:#1}}
\newcommand{\refobj}[1]{Objective~\ref{Obj:#1}}
\newcommand{\refitm}[1]{(\ref{Itm:#1})}
\newcommand{\refcon}[1]{(\ref{Con:#1})} % conclusion


==> header_basic.tex <==
%%% header_basic.tex

%%% When in doubt try to err on the side of writing more in
%%% the tex file than in the header material -- thus, hopefully, the
%%% tex file will make mathematical sense even if the header file
%%% goes missing.

%%% Packages %%%

\usepackage{amsmath} %%% Defines \numberwithin, \operatorname
\usepackage{amssymb} %%% Defines \mathbb
\usepackage{amsthm} %%% Defines \theoremstyle

\usepackage{microtype} 
%\usepackage[protrusion=true,expansion=false]{microtype} 
\usepackage{pinlabel} 

% Hyperref -- common advice seems to be ``put hyperref last''.
% see http://www.tug.org/applications/hyperref/manual.html

\usepackage[
hidelinks,
pagebackref,
pdftex]{hyperref}

%%% Note that hidelinks replaces some version of the options:
%pdfborderstyle={},
%pdfborder={0 0 0},
%For example see:
%http://tex.stackexchange.com/questions/823/
%remove-ugly-borders-around-clickable-crossreferences-and-hyperlinks 

\renewcommand{\backreftwosep}{\backrefsep}
\renewcommand{\backreflastsep}{\backrefsep}
\renewcommand*{\backref}[1]{}
\renewcommand*{\backrefalt}[4]{
  \ifcase #1 
  [No citations.]
  \or [#2]
  \else [#2]
  \fi }

%%% Remark: it may be a good idea create a boolean variable to control
%%% compilation for viewing the output on the screen versus on paper.
%%% Basically, want to turn off the colors when printing hard copy.
%%% Perhaps use the ifthen package to do this...

%%% Remark: hypersetup doesn't work at Rutgers

%\hypersetup{
%ps2pdf,
%colorlinks=true,
%linkcolor=blue,
%citecolor=darkgreen,
%urlcolor=magenta
%}

%%% Unused commands for hyperref
%pdfborderstyle={},
%ps2pdf,
%pagebackref
%colorlinks=true
%linkcolor=blue
%citecolor=darkgreen
%urlcolor=magenta

%%% backref/pagebackref option adds page numbers to the bibliography -
%%% Very useful for hard copy (as with index).  Much faster than
%%% searching when using screen... 

%\usepackage[hyperpageref]{backref}

%\hypersetup
%pdfborderstyle={},     %%% perhaps required by the ArXiv - web says
   %this doesn't work.
%debug=true,
%pdfborder={0 0 0},     %%% trying to deal with the stupid boxes
%dvips,                 %%% driver?
%ps2pdf,                %%% driver
%hdvips,                %%% driver
%linkbordercolor={0 0 1},%          %%% blue frames around links
%pdfborder={0 0 112.0},% 
%bookmarks=true,%                   %%% generate bookmarks ...
%bookmarksnumbered=true,%           %%% ... with numbers
%hypertexnames=false,%              %%% needed for correct links to figures 
%breaklinks=true,%                  %%% breaks lines, but links are very small

% Unused packages.
%\usepackage{epsfig} 
%\usepackage{color}
%\definecolor{darkgreen}{rgb}{0, 0.40, 0}
%\usepackage{psfrag} 
% \usepackage{graphics}
% \usepackage{latexsym}
% \usepackage{verbatim} 
% \usepackage{makeidx}  %%% For making an index.  For an example of
                        %%% usage, see thesis. 

%%% New commands %%%

%%% Typographic %%%

%%% From http://tex.stackexchange.com/questions/2607/spacing-around-left-and-right
\let\originalleft\left
\let\originalright\right
\renewcommand{\left}{\mathopen{}\mathclose\bgroup\originalleft}
\renewcommand{\right}{\aftergroup\egroup\originalright}

%%% Latin

%%% Remark -- style manuals differ on whether or not abbreviations of
%%% foreign words should be italicized.  However most agree that the
%%% extra punctuation is required.  Try to avoid using these, in any
%%% case. 
\newcommand{\etc}{{\it etc}}
\newcommand{\ie}{{\it ie}}
\newcommand{\eg}{{\it eg}}
\newcommand{\etal}{{\it et\thinspace al}}
\newcommand{\sic}{{\it sic}}
\newcommand{\apriori}{{\it a\thinspace priori}}

\newcommand{\thsup}{{\rm th}}
\newcommand{\stsup}{{\rm st}}

%%% General

\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}

%\renewcommand{\AA}{\mathbb{A}} %%% Wow, this is probably a bad idea!
%Only use renewcommand if you absolutely understand what you are
%replacing... 
\newcommand{\Ann}{\mathbb{A}}
\newcommand{\BB}{\mathbb{B}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\DD}{\mathbb{D}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\FF}{\mathbb{F}}
\newcommand{\GG}{\mathbb{G}}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\KK}{\mathbb{K}}
\newcommand{\MM}{\mathbb{M}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\OO}{\mathbb{O}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
%\renewcommand{\SS}{\mathbb{S}} 
\newcommand{\Sph}{\mathbb{S}} 
\newcommand{\TT}{\mathbb{T}}
\newcommand{\VV}{\mathbb{V}}
\newcommand{\WW}{\mathbb{W}}
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\ZZ}{\mathbb{Z}}

%%% Computer Science %%%

\newcommand{\PTIME}{{\bf P}}
\newcommand{\NP}{{\bf NP}}
\newcommand{\coNP}{{\bf coNP}}
\newcommand{\PSPACE}{{\bf PSPACE}}
\newcommand{\EXPTIME}{{\bf EXPTIME}}

%%% Standard Math %%%

%%% Kasra Rafi notation
\newcommand{\emul}{\overset{.}{\asymp}}
\newcommand{\gmul}{\overset{.}{\succ}}
\newcommand{\lmul}{\overset{.}{\prec}}
\newcommand{\eadd}{\overset{+}{\asymp}}
\newcommand{\gadd}{\overset{+}{\succ}}
\newcommand{\ladd}{\overset{+}{\prec}}

%\renewcommand{\setminus}{{\smallsetminus}}

%%% functions should look like
%%% \newcommand{\diag}{\operatorname{diag}}

\newcommand{\lcm}{\operatorname{lcm}}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\proj}{\operatorname{proj}}
\newcommand{\image}{\operatorname{image}}
\newcommand{\domain}{\operatorname{domain}}
\newcommand{\Id}{\operatorname{Id}}

\newcommand{\supp}{\operatorname{supp}} % support

\newcommand{\curl}{\operatorname{curl}}
%\newcommand{\div}{\operatorname{div}}
\newcommand{\grad}{\operatorname{grad}}
\newcommand{\del}{\nabla} % gradient

\newcommand{\Vol}{\operatorname{Vol}}
\newcommand{\Area}{\operatorname{Area}}

\newcommand{\st}{\mathbin{\mid}} %%% \mathbin = binary operator,
\newcommand{\from}{\colon} % As in ``f maps _from_ X _to_ Y''.

\newcommand{\nin}{\mathbin{\notin}}

\newcommand{\defeq}{\mathrel {\mathop:}= } 
%\newcommand{\eqdef}{\mathrel {\mathop=}: } 
\newcommand{\eqdef}{=\mathrel{\mathop:}}

%%% \def\defeq{\mathbin{:=}}  %%% scary!  
%%% \newcommand{\defeq}{{\coloneqq}}  %%% Needs a package?

%%% Linear algebra

\newcommand{\ii}{{\bf i}}
\newcommand{\jj}{{\bf j}}
\newcommand{\kk}{{\bf k}}

\newcommand{\rr}{{\bf r}}
\newcommand{\uu}{{\bf u}}
\newcommand{\vv}{{\bf v}}
\newcommand{\ww}{{\bf w}}

%%% Graph Theory %%%
\newcommand{\val}{\operatorname{val}} % valency
%\newcommand{\deg}{\operatorname{deg}} % degree

%%% Topological %%%

% Relations
\newcommand{\isotopic}{\mathrel{\approx}}
\newcommand{\homeo}{\mathrel{\cong}} % Homeomorphism
\newcommand{\nhomeo}{\mathrel{\not\cong}}
\newcommand{\isom}{\cong} % Isomorphism
%\newcommand{\isom}{\mathrel{\cong}} % Isomorphism
\newcommand{\disjoint}{\mathbin{\sqcup}} % Disjointness
\newcommand{\cross}{\times}
\newcommand{\cutby}{\mathbin{\rule[.023 in]{.12 in}{.02 in}}} 

\newcommand{\free}{\mathbin{\ast}}

\newcommand{\bdyrel}[2]{\overline{\bdy{#1} \setminus \bdy{#2}}}

% Functions
\newcommand{\cover}[1]{{\widetilde{#1}}}
\newcommand{\double}[1]{{\mbox{Doub}({#1})}}
\newcommand{\lift}[1]{{\widetilde{#1}}}
\newcommand{\closure}[1]{{\overline{#1}}}
%\newcommand{\bar}[1]{{\overline{#1}}}

\newcommand{\euler}{\operatorname{\chi}} % Euler characteristic
\newcommand{\neigh}{\operatorname{neigh}} % Open regular neighborhood
\newcommand{\Neigh}{\closure{\neigh}} % Closed regular neighborhood
%%%\newcommand{\neigh}{\operatorname{\eta}} % Open regular neighborhood
%%%\newcommand{\Neigh}{\closure{\neigh}} % Closed regular neighborhood
\newcommand{\frontier}{\operatorname{fr}} 
\newcommand{\fr}{\operatorname{fr}} % Frontier
\newcommand{\bdy}{\partial} % Boundary
\newcommand{\rel}{\operatorname{rel}} % relative
\newcommand{\dual}{\operatorname{dual}} 
\newcommand{\link}{\operatorname{link}}

\newcommand{\diam}{\operatorname{diam}} % diameter

\newcommand{\vol}{\operatorname{vol}}
\newcommand{\genus}{\operatorname{genus}}
\newcommand{\interior}{{\operatorname{interior}}}
\newcommand{\connect}{\#} % Connected sum

\newcommand{\Deck}{{\operatorname{Deck}}}

% Spaces
\newcommand{\RP}{\mathbb{RP}} % real projective space
\newcommand{\QP}{\mathbb{QP}} % rational projective space
\newcommand{\CP}{\mathbb{CP}} % complex projective space
\newcommand{\pt}{\rm pt} % Point

% Groups

\newcommand{\Stab}{\operatorname{Stab}}

\newcommand{\Mod}{\operatorname{Mod}} % Modular group
\newcommand{\MCG}{\mathcal{MCG}} % Mapping class group
\newcommand{\Homeo}{\operatorname{Homeo}} % Homeomorphism group
\newcommand{\Isom}{\operatorname{Isom}} % Isometry or isomorphism group

\newcommand{\Aut}{\operatorname{Aut}} % Automorphism group
\newcommand{\Out}{\operatorname{Out}} % Outer automorphism group
\newcommand{\Inn}{\operatorname{Inn}} % Inner automorphism group

%\newcommand{\GL}{\operatorname{GL}} % General linear
\newcommand{\SL}{\operatorname{SL}} % Special linear
\newcommand{\PGL}{\operatorname{PGL}} % Projective general linear
\newcommand{\PSL}{\operatorname{PSL}} % Projective special linear
\newcommand{\SO}{\operatorname{SO}} % Special orthogonal
\newcommand{\Sp}{\operatorname{Sp}} % Symplectic

% Thurstonia %
\newcommand{\MF}{\mathcal{MF}} % Measured foliations
\newcommand{\PMF}{\mathcal{PMF}} % Projectivize

\newcommand{\GL}{\mathcal{GL}} % Geodesic laminations
\newcommand{\ML}{\mathcal{ML}} % Measured laminations
\newcommand{\PML}{\mathcal{PML}} % Projectivize
\newcommand{\FL}{\mathcal{FL}} % Filling laminations
\newcommand{\EL}{\mathcal{EL}} % Ending laminations

\newcommand{\QF}{\mathcal{QF}}  % Quasi-Fuchsian space
\newcommand{\Teich}{{Teichm\"uller~}} 

\newcommand{\Ext}{\operatorname{Ext}} % Extremal length

% For comments -- but didn't work very well.
%\newsavebox{\savepar}
%\newenvironment{boxit}{\begin{lrbox}{\savepar}
%        \begin{minipage}[b]{4.5in}}
%        {\end{minipage}\end{lrbox}\fbox{\usebox{\savepar}}}

\newcommand{\twist}{\mathrel{%
    \stackrel{\sim}{\smash{\times}\rule{0pt}{0.6ex}}
    }} % twisted product

\newcommand{\quotient}[2]{{\raisebox{0.2em}{$#1$}
           \!\!\left/\raisebox{-0.2em}{\!$#2$}\right.}}


==> header_subtle.tex <==
%%% Weird proof environments (to get qedboxes like WPiG)

%% \newcommand{\qbox}[1]{
%%     \setlength\fboxsep{2pt} % should be a percentage, not fixed 
%%     \fbox{\small{\ref{#1}}}
%% }

%% \newenvironment{qproof}[1]{
%%   \def\tempname{#1}
%%   \noindent{\it Proof \ref{#1}.}
%% }{
%%   \hfill\qbox{\tempname}
%% }

%% \newenvironment{qqproof}[2][\proofname]{
%%   \def\tempname{#2}
%%   \noindent{\it #1.}
%% }{
%%   \hfill\qbox{\tempname}
%% }

%%% other ideas:
%%% [\tempname] or \makebox{\tempname}
%\newlength{\wpflen}  % outside
%%% Try to import proof env from amsart.cls... ??
%%%  \settowidth{\wpflen}{\fbox{\small{\tempname}}} % inside
%%%  \hfill\parbox[b]{\wpflen}{\fbox{\small{\tempname}}}%\vspace{1ex}

%%% Fake environments 

%%% Old 
%\newcommand{\head}[1]{{\vspace{0.5\baselineskip} \noindent {\bf #1.}}}
%%% This causes various spacing problems.  Perhaps replace by
%%% subsubsection*? or some such...

%%% New
%%% The code below was copied from 
%%% http://groups.google.com/group/comp.text.tex/browse_frm/
%%% thread/97fefc09a54fa5df/49f1ad7d5cefd902#49f1ad7d5cefd902

%
\newcommand{\fakeenv}{} %%% prints the emptystring

%%% For theorem style
\newenvironment{restate}[2]  %%% restate takes two arguments 
{ 
 \renewcommand{\fakeenv}{#2} %%% So now \fakeenv prints #2
 \theoremstyle{plain} 
 \newtheorem*{\fakeenv}{#1~\ref{#2}} %%% so now #2 is the name of a
                                     %%% theorem-like environment.   
 \begin{\fakeenv}
}
{
 \end{\fakeenv}
}

%%% For definition style 
\newenvironment{restated}[2]  
{ 
 \renewcommand{\fakeenv}{#2} 
 \theoremstyle{definition} 
 \newtheorem*{\fakeenv}{#1~\ref{#2}} %%% so now #2 is the name of a
                                     %%% definition-like environment.   
 \begin{\fakeenv}
}
{
 \end{\fakeenv}
}

%%% Example of usage of restate

%%% Somewhere there is a theorem ---
%%%
%%% \begin{theorem}[Wiles]
%%% \label{Thm:Main}
%%% For $n \geq 3$ there are no non-trivial integer solutions to:
%%% \[ x^n + y^n = z^n. \]
%%% \end{theorem}
%%%
%%% and somewhere it is repeated. 
%%% 
%%% \begin{restate}{Theorem}{Thm:Main}[Wiles]
%%% The equation $x^n + y^n = z^n$ has only trivial solutions over
%%% the integers. 
%%% \end{restate}

%%% In practice I have the restatement early (eg in the first section)
%%% and the actual theorem late.

%%% A slightly tricky point: you can't use restate twice for the
%%% _same_ theorem because eg, \renewtheorem doesn't work.  But this 
%%% isn't a problem.  The second+ time you want to restate Thm:Foo
%%% just type 
%%% \begin{Thm:Foo} and \end{Thm:Foo} and everything works.  Groovy.

%%% takes 1) Hint/Solution 2) the label 3) exercise and 4) hint or
%%% solution and then prints the exercise where it is and prints the
%%% hint at the end.  
\newcommand{\exercisewith}[4]{
  \begin{exercise}
  \label{#2}
  #3
  \end{exercise}
  \AtEndDocument
  {
    \begin{restated}{#1}{#2}
    #4    
    \end{restated}
  }
}
%%% Perhaps more elegant to use the answer package... 
%%% Ask on the tex.stackexchange site?

%%% Here is what I want: 
%%% \exercise{Ex:Fermat}
%%% {Show that there are no positive integer solutions to $x^n + y^n =
%%% z^n$, when $n > 2$.}
%%% {Try to find a useful elliptic curve, a la~\cite{Frey86}.}
%%% {I have found a truly wonderful proof, but this solution
%%% environment is too small to contain it. Instead,
%%% see~\cite{Wiles95}.}


